Machine Unlearning via Algorithmic Stability

We study the problem of machine unlearning and identify a notion of algorithmic stability, Total Variation (TV) stability, which we argue, is suitable for the goal of exact unlearning. For convex risk minimization problems, we design TV-stable algorithms based on noisy Stochastic Gradient Descent (SGD). Our key contribution is the design of corresponding efficient unlearning algorithms, which are based on constructing a (maximal) coupling of Markov chains for the noisy SGD procedure. To understand the trade-offs between accuracy and unlearning efficiency, we give upper and lower bounds on excess empirical and populations risk of TV stable algorithms for convex risk minimization. Our techniques generalize to arbitrary non-convex functions, and our algorithms are differentially private as well.

==> sections/proofsruntime.tex <==
\section{Proofs for \cref{sec:runtime}}
\label{sec:proofs-runtime}
\begin{proof}[Proof of Proposition \ref{prop:runtime_main}]
We first setup some notation. 
In the general setup, for $k$ edit requests, let $s$ be the number of times a recompute is triggered. 
Let $\bc{Z_1,Z_2,\ldots, Z_s}$ be a set of random variables, where each $Z_i$ denotes how many edit requests the $i^{\text{th}}$ recompute can \emph{handle}. 
To elaborate, $Z_i$ takes value $j$, if upon $j$ edit requests, a recompute is triggered. 
The $Z_i$'s comprises to the randomness used in the algorithm like mini-batching indices or Gaussian noise, as well as the randomness used for rejection sampling.
% The $Z_i$'s correspond to the randomness used in the batch algorithm which aids unlearning, like mini-batching indices or Gaussian noise. 
% Moreover, since we stop the algorithm and trigger a recompute once we have seen $1+\frac{1}{\rho}$ requests, we also have that $Z_i \leq 1+\frac{1}{\rho}$. Hence, we have $Z_i \leq \min \br{k,1+\frac{1}{\rho}}$. Therefore in the regime where $1+\frac{1}{\rho}\geq k \iff \rho \leq \frac{1}{k-1}$, this condition is inactive, as it means that we have seen all $k$ requests before the external recompute trigger.
It is important to note that $Z_i's$ are not necessarily independent. 
In particular, in Algorithm \ref{alg:unlearn-noisy-m-a-sgd}, we reuse the Gaussian noise upto the iteration in which rejection sampling fails, and only use fresh/independent Gaussian noise in the later steps.
However, note that we have exact unlearning, and the output at each step is $\rho$-TV stable (w.r.t. all the randomness used). Hence, since the above description of the distribution of $Z_i$'s depend only on the TV stability parameter,
it follows that $Z_i's$ are (marginally) identical.
% Finally, since upon each recompute, we use independent randomness, all $Z_i$'s are independent. 

% We now use the $\rho$-Total Variation property of the algorithm, as well as maximal coupling to describe the probability distribution of $Z_i$. 
We now use the fact that the unlearning algorithm constructs a coupling with acceptance probability at least $1-\rho$ to describe the probability distribution of $Z_i$. 
We have that upon one edit request, the probability that a recompute is triggered is at most $\rho$. 
This means that $Z_i < 2$ with probability $\leq \rho$. 
Using Remark \ref{remark:tv_upto_k}, this generalizes as $Z_i < j$ with probability at most $(j-1)\rho$.
Note that in our setup, we observe at most $k$ requests, so $Z_i$ taking values larger than $k$ is not meaningful. However if $k\rho < 1$, it means that probability that $Z_i$ takes values smaller than $k$ is less than $1$, and therefore there is a positive probability of $Z_i$ being larger than $k$. 
To remedy this, we define another random variable $X_i$'s which takes values in the set $\bc{1,2,\ldots, k}$. 
Furthermore, for any $i$,  $\P{X_i = j} = \P{Z_i = j}$ for $j\leq k$, but $\P{Z_i = j} = \sum_{l=k}^\infty \P{X_i=l}$. By construction, this ensures that $1\leq Z_i\leq k$, when we observe at most $k$ requests. 


% This step is done only for theoretical purposes, and the algorithm would actually benefit if it were not done.


We want upper bounds on $s$ conditioned on the fact that $k$ requests are addressed i.e. $X_1+X_2 \ldots, X_s \geq k$. 
% For this we write $s$ as $s:=\min_q\bc{k+ \br{1+\frac{1}{\rho}} \geq X_1+X_2 \ldots, X_q \geq k}$.
For this we write $s$ as $s:=\min_q\bc{2k \geq X_1+X_2 \ldots, X_q \geq k}$. 
The first inequality holds trivially since we ensured that $X_i\leq k$.
% we stop the algorithm upon $\br{1+\frac{1}{\rho}}$ requests without recompute. 
It is easy to see that $s$ is a stopping time with respect to the filtered probability space of the stochastic process $\bc{X_i}_{i\in \bbN}$. 
Furthermore, since $X_i$'s are identical, we can apply Wald's equation to get,
% \begin{align*}
%      &k + \br{1+\frac{1}{\rho}} \geq \mathbb{E}[X_1+X_2 + \ldots, X_s] = \mathbb{E}[s] \mathbb{E}X_1] =  \mathbb{E}[s]  \sum_{j=1}^{1+1/\rho} \bbP\bc{X_i \geq j}  \\&=  \mathbb{E}[s]  \sum_{j=1}^{1+1/\rho}\br{1- \bbP\bc{X_i < j}} \geq   \mathbb{E}[s]\br{\frac{1}{\rho} - \sum_{j=1}^{1+1/\rho}(j-1)\rho} \geq  \mathbb{E}[s]\br{\frac{1}{\rho} - \int_{j=0}^{1/\rho}j\rho dj}  \\& \geq \mathbb{E}[s]\br{\frac{1}{\rho} - \frac{1}{2\rho^2}\rho} 
%      \geq  \frac{\mathbb{E}[s]}{2\rho}
%         % }
% \end{align*}
\begin{align*}
     &2k \geq \mathbb{E}[X_1+X_2 + \ldots X_s] = \mathbb{E}[s] \mathbb{E}[X_1] =  \mathbb{E}[s]  \sum_{j=1}^{k} \bbP\bc{X_i \geq j} =
      \mathbb{E}[s]  \sum_{j=1}^{\infty} \bbP\bc{Z_i \geq j} 
     \\& \geq \mathbb{E}[s]  \sum_{j=1}^{1+1/\rho} \bbP\bc{Z_i \geq j}  =  \mathbb{E}[s]  \sum_{j=1}^{1+1/\rho}\br{1- \bbP\bc{Z_i < j}} \geq   \mathbb{E}[s]\br{\frac{1}{\rho} - \sum_{j=1}^{1+1/\rho}(j-1)\rho} \\&\geq  \mathbb{E}[s]\br{\frac{1}{\rho} - \int_{j=0}^{1/\rho}j\rho dj}   \geq \mathbb{E}[s]\br{\frac{1}{\rho} - \frac{1}{2\rho^2}\rho} 
     \geq  \frac{\mathbb{E}[s]}{2\rho}
        % }
\end{align*}
This gives us that $\mathbb{E}[s] \leq 4k\rho$. 
% This result is in the setting that $\rho\leq 1$
% + 2\rho + 2 \leq 6k\rho$
\end{proof}

\begin{proof}[Proof of \cref{claim:runtime_sub_sample_GD}]
The total runtime of Algorithm \ref{alg:unlearn-subsample-gd} is the time for verification plus the runtime for recomputation, whenever a recompute is triggered. 
The recomputation time is just the training time, and in the model considered, excepted cost of one recomputation takes $O\br{T m \br{\mathfrak{G}+d}}$ time, since at every iteration, $m$ gradients are computed and vectors added. 
% $O\br{\frac{T \br{\frac{n}{m}\mathfrak{G}+d)}{n}}$ time
% - this is because at every iteration, $m$ gradients are computed and vectors added. 
As discussed in \cref{sec:runtime}, the expected verification time for Algorithm \ref{alg:unlearn-subsample-gd} is $O(1)$. 
From \cref{prop:unlearn-subsample-GD}, the unlearning \cref{alg:unlearn-subsample-gd} recomputes with probability $O(\min\bc{\rho,1})$ for one edit request.
Therefore, using Proposition \ref{prop:runtime_main} which bounds the number of recomputes, we have that the expected total runtime is bounded as $kO(1) + 4k\min\bc{\rho,1} \cdot O\br{T m \br{\mathfrak{G}+d}} \leq O\br{\max\br{1, \min\bc{\rho,1}T m \br{\mathfrak{G}+d}}k}$.
For a sufficiently large $\rho$, the unlearning time of Algorithm \ref{alg:unlearn-subsample-gd} is clearly dominated by the training time. 
In particular, in the corresponding batch Algorithm \ref{alg:sub-sample-GD}, we set $m=\frac{\rho n}{T}$, giving a total runtime of $O\br{\max\br{1, \min\bc{\rho^2,1}n \br{\mathfrak{G}+d}}k}$. 
%  this gives us that the total runtime time is $O\br{\max\br{1, \rho^2 n \br{\mathfrak{G}+d}}k}$. 
Hence for $\rho \gtrsim \frac{1}{\sqrt{n(\mathfrak{G}+d})}$, the total runtime in expectation is at most $O(\min\bc{\rho,1} \cdot k\cdot \text{Training time})$. 
In the other case, the expected total runtime is just $O(k)$.
\end{proof}

\begin{proof}[Proof of \cref{claim:runtime_noisy_A_SGD}]
As before, the total runtime of Algorithm \ref{alg:unlearn-subsample-gd} is the time for verification plus the runtime for recomputation, whenever a recompute is triggered. 
As discussed in \cref{sec:runtime}, the expected verification time for Algorithm \ref{alg:unlearn-noisy-m-a-sgd} is $O\br{\frac{Tm(\mathfrak{G}+d)}{n}}$. 
The recomputation in this case may be partial but it also includes a reflection.
The reflection operation with $d$ dimensional vectors takes $O(d)$ compute. 
Furthermore, we upper bound the partial recomputation time by worst-case full recomputation time, giving a recomputation time of
% - this gives us that 
% the recomputation time is 
$O\br{T m \br{\mathfrak{G}+d}}$.
From \cref{lem:noisy-m-sgd-accept}, we have that the unlearning coupling is not maximal but recomputes with probability $\min\bc{\rho \sqrt{T},1}$.
Finally, by Proposition \ref{prop:runtime_main} we have that the expected total runtime is bounded as $kO\br{T m \br{\mathfrak{G}+d}} + 4k\min\bc{\rho \sqrt{T},1} \cdot O\br{ \frac{Tm(\mathfrak{G}+d)}{n}} \leq O\br{\max\br{\min\bc{\rho \sqrt{T},1},\frac{1}{n}}kmT(\mathfrak{G}+d)}$.
In contrast, for Algorithm \ref{alg:unlearn-noisy-m-a-sgd}, the runtime is at most $O\br{\max\br{\min\bc{\rho \sqrt{T},1},\frac{1}{n}}kmT(\mathfrak{G}+d)}$. 
Our lower bounds will show that we need $\rho \gtrsim \frac{1}{n}$ to get any non-trivial accuracy.
Therefore the maximum is always obtained by $\min\bc{\rho \sqrt{T},1}$. 
Moreover, $k$ is a trivial lower bound on runtime, since we need to observe all $k$ edit requests. 
Hence, we get that the total runtime in expectation, is at most $O\br{\max\bc{k,\min\bc{\rho \sqrt{T},1}\cdot k \cdot \text{Training time}}}$. 
% Finally, using Proposition \ref{prop:runtime_main}, we have that the expected total runtime is bounded as $kO\br{T m \br{\mathfrak{G}+d}} + 4k\rho \cdot O\br{ \frac{Tm(\mathfrak{G}+d)}{n}} \leq O\br{\max\br{\rho,\frac{1}{n}}kmT(\mathfrak{G}+d)}$.
\end{proof}
